Skill Transfer and Discovery for Sim-to-Real Learning: A Representation-Based Viewpoint

We study sim-to-real skill transfer and discovery in the context of robotics control using representation learning. We draw inspiration from spectral decomposition of Markov decision processes. The spectral decomposition brings about representation that can linearly represent the state-action value function induced by any policies, thus can be regarded as skills. The skill representations are transferable across arbitrary tasks with the same transition dynamics. Moreover, to handle the sim-to-real gap in the dynamics, we propose a skill discovery algorithm that learns new skills caused by the sim-to-real gap from real-world data. We promote the discovery of new skills by enforcing orthogonal constraints between the skills to learn and the skills from simulators, and then synthesize the policy using the enlarged skill sets. We demonstrate our methodology by transferring quadrotor controllers from simulators to Crazyflie 2.1 quadrotors. We show that we can learn the skill representations from a single simulator task and transfer these to multiple different real-world tasks including hovering, taking off, landing and trajectory tracking. Our skill discovery approach helps narrow the sim-to-real gap and improve the real-world controller performance by up to 30.2%.

==> content/introduction.tex <==
\section{Introduction}
% Reinforcement learning (RL) has demonstrated superior performance in many strategic games and robotic simulators\cite{silver_mastering_2017,wurman_outracing_2022}. 
Sim-to-real transfer, i.e., transferring the policy learned in simulators to real-world robots,  has long been a very challenging question in the robot learning community. One of the difficulties is that the simulator can never capture the exact real-world dynamics. For example, the simulator cannot precisely capture the real-world noise, physical parameters, contact effects, signal and response delays, package losses, etc. The differences between simulator and real-world dynamics are called the residual dynamics. 



% The most commonly used sim-to-real transfer technique is domain randomization \cite{tobin_domain_2017}, where the physical parameters of the simulators are randomly selected 

% There are multiple reasons that sim-to-real transfer is challenging. For example, the noisy real-world observations, and differences in transition dynamics between the simulator and real world, xxx. In this paper, we will focus on the problem of learning the sim-to-real gap, or the residual dyanmics learning. Moreover, we consider that the real-world data is expensive to get. (expensive compared to the simulators). We would like to design a sample-efficient algorithm to transfer the knowledge learned in the simulators to the real world.

% The most commonly used method to tackle the differences in dynamics should be domain randomization \cite{tobin_domain_2017}. Domain randomization in robotics usually means that the simulator randomly generates physical parameters in the dynamics model, rather than using only one specific dynamics. For example, \citet{andrychowicz_learning_2020} randomize the mass, friction and damping coefficients, 

Learning the residual dynamics appears in many recent sim-to-real transfer studies \cite{levine_learning_2014,saveriano_data-efficient_2017,kaufmann_champion-level_2023}. The major challenge of residual dynamics learning is that the real-world data is expensive. Therefore, sample-efficient models are preferred. 
Existing practices of residual dynamics learning have considered Gaussian mixture model~\cite{levine_learning_2014}, Gaussian process \cite{saveriano_data-efficient_2017,fisac_general_2019} or k-nearest neighbors \cite{kaufmann_champion-level_2023}. 
% However, these methods usually learn the residual dynamics as a separate model learning problem, leaving the rich simulator information unused. Moreover, these methods usually put strict assumptions on the dynamics structure that restricts the learning capabilities on complex residual dynamics. 

Recent studies in the theoretical RL community on low-rank Markov decision processes (MDP), or linear MDPs,  \cite{jin_provably_2019,agarwal_flambe_2020} reveal another sample-efficient approach to learning the transition dynamics and then the control policies. 
The low-rank structure of MDPs assumes that there exists low-rank decompositions of the transition dynamics. This low-rank strcuture allows that the state-action value function (the Q-function) with any policy could be \textit{linearly} represented with a finite set of function bases. These bases are also called the low-rank \emph{representations}. Therefore, if the representations are known, the planning tasks reduce to. Moreover, if the representations are not known, we can also learn the representation in a sample-efficient way using maximum likelihood estimation (MLE) or SVD decomposition \cite{uehara_representation_2022,ren_spectral_2023,ren_latent_2023}.

Inspired by the sample-efficient low-rank MDPs, we proposed a xxx algorithm in this paper leveraging representation learning to learn the residual dynamics. \todo{Improve the writing here.} simply applying the existing representation learning techniques to the residual dynamics learning, we encourage the residual dynamics representation orthogonal to simulator dynamics representations. This orthogonality further leverages simulator information to help residual dynamics learning \todo{But residual dynamics itself also somehow use the simulator information?}
Moreover, compared to residual RL that only returns the policy, we can explicitly learn the residual dynamics model that can help improve the simulators to be more realistic. We show the transfer learning on real quadcoptors. \todo{add exp results.} According to our knowledge, this is the first paper applying linear/low-rank MDP results on real-world robots.

% Intuitively speaking, we assume that we can have a low-rank decomposition of the dynamics. Then we can linearly represent the state-action value function (Q-functions) \emph{for any policy} with the decomposition results. Therefore, sample-efficient planning is possible because we only optimize the linear weights of the representations.

% the decomposition is also called the low-rank representation of 

% The decomposition results serve as a representation which allows us to learn a set of basis of the state-action value function (the Q-function). 

% In this paper, we leverage this representation learning scheme to show the sample-efficient representation learning for sim-to-real transfer. First, we can easily adapt the weights. Moreover, as the Q function induced by the real-world model might not lie in the same function space spanned by previous function basis, we use the representation learning techniques to learn additional basis to augment and enlarge the function space. 



% To tackle the problem, we proposed a xxx algorithm to learn the residual dynamics. 


% We got inspiration from the low-rank Markov decision process (MDP) studies , where we assume that the transition dynamics $P(s'\mid s, a)$ \todo{handle the notation} could be decomposed as $P(s'\mid s, a) = \left\langle\phi(s,a),\mu(s')\right\rangle$. In this way, we can represent The state-action value function as a linear combination of $\phi(s, a)$, which means we know the basis of function Q. If we know the function basis $\phi(s, a)$, then we only need to find weights $w$ to search for the optimal policy. Recent studies also discussed representation learning methods \cite{uehara_representation_2022, ren_spectral_2023} when the representation $\phi$ is not known.  

==> fig/tikz_block_1.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300


% Text Node
\draw    (7.83,127.25) .. controls (7.83,125.59) and (9.18,124.25) .. (10.83,124.25) -- (75.83,124.25) .. controls (77.49,124.25) and (78.83,125.59) .. (78.83,127.25) -- (78.83,146.25) .. controls (78.83,147.91) and (77.49,149.25) .. (75.83,149.25) -- (10.83,149.25) .. controls (9.18,149.25) and (7.83,147.91) .. (7.83,146.25) -- cycle  ;
\draw (10.83,128.25) node [anchor=north west][inner sep=0.75pt]   [align=left] {Simulator};
% Text Node
\draw    (121.5,127.75) .. controls (121.5,126.09) and (122.84,124.75) .. (124.5,124.75) -- (168.5,124.75) .. controls (170.16,124.75) and (171.5,126.09) .. (171.5,127.75) -- (171.5,145.75) .. controls (171.5,147.41) and (170.16,148.75) .. (168.5,148.75) -- (124.5,148.75) .. controls (122.84,148.75) and (121.5,147.41) .. (121.5,145.75) -- cycle  ;
\draw (124.5,129.15) node [anchor=north west][inner sep=0.75pt]    {$RL( \alpha )$};
% Text Node
\draw    (219.65,116.25) .. controls (219.65,114.59) and (221,113.25) .. (222.65,113.25) -- (318.65,113.25) .. controls (320.31,113.25) and (321.65,114.59) .. (321.65,116.25) -- (321.65,157.25) .. controls (321.65,158.91) and (320.31,160.25) .. (318.65,160.25) -- (222.65,160.25) .. controls (221,160.25) and (219.65,158.91) .. (219.65,157.25) -- cycle  ;
\draw (222.65,117.25) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{66.77pt}\setlength\topsep{0pt}
Control output
\begin{center}
$\displaystyle u$
\end{center}

\end{minipage}};
% Text Node
\draw    (394.19,127.25) .. controls (394.19,125.59) and (395.53,124.25) .. (397.19,124.25) -- (470.19,124.25) .. controls (471.85,124.25) and (473.19,125.59) .. (473.19,127.25) -- (473.19,146.25) .. controls (473.19,147.91) and (471.85,149.25) .. (470.19,149.25) -- (397.19,149.25) .. controls (395.53,149.25) and (394.19,147.91) .. (394.19,146.25) -- cycle  ;
\draw (397.19,128.25) node [anchor=north west][inner sep=0.75pt]   [align=left] {Real world};
% Text Node
\draw    (548.15,115.25) .. controls (548.15,113.59) and (549.5,112.25) .. (551.15,112.25) -- (639.15,112.25) .. controls (640.81,112.25) and (642.15,113.59) .. (642.15,115.25) -- (642.15,156.25) .. controls (642.15,157.91) and (640.81,159.25) .. (639.15,159.25) -- (551.15,159.25) .. controls (549.5,159.25) and (548.15,157.91) .. (548.15,156.25) -- cycle  ;
\draw (551.15,116.25) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{61.08pt}\setlength\topsep{0pt}
Performance
\begin{center}
$\displaystyle J( \alpha )$
\end{center}

\end{minipage}};
% Text Node
\draw (175,117.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small unroll}};
% Text Node
\draw (83,117.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small train}};
% Text Node
\draw (5,82.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \alpha $: simulator parameters};
% Text Node
\draw (249,219.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{118.15pt}\setlength\topsep{0pt}
\begin{center}
differentiable optimization\\(gradient descent)
\end{center}

\end{minipage}};
% Text Node
\draw (326,117.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small implement}};
% Text Node
\draw (479,117.83) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small evaluate}};
% Connection
\draw    (78.83,136.75) -- (119.5,136.75) ;
\draw [shift={(121.5,136.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (171.5,136.75) -- (217.65,136.75) ;
\draw [shift={(219.65,136.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (321.65,136.75) -- (392.19,136.75) ;
\draw [shift={(394.19,136.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (473.19,136.51) -- (546.15,136.05) ;
\draw [shift={(548.15,136.04)}, rotate = 179.65] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (548.15,156.25) .. controls (389.96,232.47) and (230.47,230.14) .. (69.66,149.25) ;
\draw [shift={(69.66,149.25)}, rotate = 26.7] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

\end{tikzpicture}


==> fig/tikz_block_2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da7338442636547493] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (251.33,210.33) -- (320.4,210.47) ;
%Straight Lines [id:da5117884969557032] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (320.09,120.26) -- (320.4,210.47) ;
%Straight Lines [id:da6065466919863187] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (269.09,120.26) -- (320.09,120.26) ;
\draw [shift={(267.09,120.26)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp4996384200577939] 
\draw  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (9.5,47.26) .. controls (9.5,33.45) and (20.69,22.26) .. (34.5,22.26) -- (253.59,22.26) .. controls (267.39,22.26) and (278.59,33.45) .. (278.59,47.26) -- (278.59,122.26) .. controls (278.59,136.06) and (267.39,147.26) .. (253.59,147.26) -- (34.5,147.26) .. controls (20.69,147.26) and (9.5,136.06) .. (9.5,122.26) -- cycle ;
%Rounded Rect [id:dp2006102165852075] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (9.5,178.26) .. controls (9.5,164.45) and (20.69,153.26) .. (34.5,153.26) -- (253.59,153.26) .. controls (267.39,153.26) and (278.59,164.45) .. (278.59,178.26) -- (278.59,253.26) .. controls (278.59,267.06) and (267.39,278.26) .. (253.59,278.26) -- (34.5,278.26) .. controls (20.69,278.26) and (9.5,267.06) .. (9.5,253.26) -- cycle ;

% Text Node
\draw    (23.04,53.33) -- (265.04,53.33) -- (265.04,85.33) -- (23.04,85.33) -- cycle  ;
\draw (26.04,57.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {Fit $\displaystyle \phi ^{\top }( s,a)$ form simulator model $\displaystyle \hat{P}$};
% Text Node
\draw    (21.54,107) -- (266.54,107) -- (266.54,133) -- (21.54,133) -- cycle  ;
\draw (24.54,111) node [anchor=north west][inner sep=0.75pt]   [align=left] {Generate orthogonal basis $\displaystyle \bar\phi(s,a)$};
% Text Node
\draw    (36.54,160.67) -- (251.54,160.67) -- (251.54,250.67) -- (36.54,250.67) -- cycle  ;
\draw (39.54,164.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{143.54pt}\setlength\topsep{0pt}
Real world learning on $\displaystyle \{\phi ,\bar\phi\}$
\begin{center}
(Details TBD, including \\exploration strategy, \\basis selection with in $\displaystyle \bar\phi$)
\end{center}

\end{minipage}};
% Text Node
\draw (30,29) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,opacity=1 ] [align=left] {Simulator};
% Text Node
\draw (25,256) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {Real World};
% Text Node
\draw (327,156) node [anchor=north west][inner sep=0.75pt]   [align=left] {?};
% Connection
\draw    (144.04,85.33) -- (144.04,105) ;
\draw [shift={(144.04,107)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% Connection
\draw    (144.04,133) -- (144.04,158.67) ;
\draw [shift={(144.04,160.67)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

\end{tikzpicture}

